PixL2R: Guiding Reinforcement Learning Using Natural Language by Mapping Pixels to Rewards

Reinforcement learning (RL), particularly in sparse reward settings, often requires prohibitively large numbers of interactions with the environment, thereby limiting its applicability to complex problems. To address this, several prior approaches have used natural language to guide the agent's exploration. However, these approaches typically operate on structured representations of the environment, and/or assume some structure in the natural language commands. In this work, we propose a model that directly maps pixels to rewards, given a free-form natural language description of the task, which can then be used for policy learning. Our experiments on the Meta-World robot manipulation domain show that language-based rewards significantly improves the sample efficiency of policy learning, both in sparse and dense reward settings.

==> bkgrd.tex <==
\section{Background}

\subsection{Markov Decision Process}

Reinforcement learning consists of an agent interacting with an environment. The learning problem is typically represented using a Markov Decision Process (MDP) $M = \langle S, A, T, R, \gamma \rangle$. Here, $S$ is the set of all states in the environment, $A$ is the set of actions available to the agent, $T : S \times A \times S \rightarrow [0, 1]$ is the transition function of the environment, $R : S \times A \rightarrow \mathds{R}$ is the reward function, and $\gamma \in [0, 1]$ is a discount factor.

At timestep $t$, the agent observes a state $s_{t} \in S$, and takes an action $a_{t} \in A$, according to some policy $\pi : S \times A \rightarrow [0, 1]$. The environment transitions to a new state $s_{t+1} \sim T(s_{t}, a_{t}, \cdot)$, and the agent receives a reward $R_{t} = R(s_{t}, a_{t})$.
The goal is to learn a policy $\pi$, such that the expected future return, $G_{t} = \sum_{t=0}^{T} \gamma^{t} R_{t}$, is maximized.

% The goal is to learn a policy $\pi$, such that the expected future return, $G_{t}$, defined as follows, is maximized:
% \[
% G_{t} = \sum_{t=0}^{T} \gamma^{t} R_{t}
% \]


In this work, we use an extension of the standard MDP, defined as $M' = \langle S, A, T, R, \gamma, L \rangle$, where $L$ is an instruction describing the task using natural language, and the other quantities are as defined above. 
% We denote this modified MDP as MDP+L (introduced by \citeauthor{goyal:ijcai19} (\citeyear{goyal:ijcai19})).

% \subsection{Prior Work: LEARN}
% \label{sec:learn}

% \citeauthor{goyal:ijcai19} (\citeyear{goyal:ijcai19}) proposed a framework for learning in an MDP+L, which consists of the following two phases. 

% \textbf{Phase 1}: A neural network -- the LanguagE Action Reward Network (LEARN) -- is trained to predict whether a given trajectory and language are related or not. This requires paired \la trajectory, language\ra data in the environment. As a preprocessing step, each trajectory is first encoded into an \textit{action frequency vector}, which is a vector of size $|A|$, with the $i^{th}$ component proportional to the number of times action $i$ appears in the trajectory.  The neural network takes this action frequency vector and language as inputs to predict the relatedness between the trajectory and language, which is modelled as a binary classification problem.

% \textbf{Phase 2}: Next, a policy is trained for a new task in the MDP+L setting -- the extrinsic reward from the environment is assumed to be sparse (i.e. 1 if the agent successfully completes the task, and 0 otherwise), and the agent additionally gets a language command describing the task. At every step, an action frequency vector is created from the sequence of past actions and passed to the pretrained LEARN model along with the given command. The LEARN model generates probabilities over classes \texttt{RELATED} and \texttt{UNRELATED}, which are used to generate intermediate rewards for reward shaping \cite{ng1999policy}.



==> tables.tex <==
\begin{table}[]
    % \caption{Global caption}
    \begin{minipage}{.58\linewidth}
      \caption{Average magnitude of gradients for different words in a description for the relatedness score prediction.}
      \centering
\resizebox{\columnwidth}{!}{
\begin{tabular}{|r|rrrrrrr|}
\hline
\multicolumn{1}{|l|}{\textbf{}} & \multicolumn{7}{c|}{\textbf{Descriptions}}              \\ 
\multicolumn{1}{|c|}{\textbf{}} & \multicolumn{7}{c|}{\textbf{Average magnitude of gradient for each word}}       \\ \hline
1.                              & push  & the  & green  & button &       &      &         \\ 
                                & 0.53  & 0.30 & 1.00   & 0.94   &       &      &         \\ \hline
2.                              & push  & down & the    & red    & block &      &         \\ 
                                & 0.42  & 0.57 & 0.34   & 1.00   & 0.91  &      &         \\ \hline
3.                              & pull  & down & the    & lever  & on    & the  & toaster \\ 
                                & 0.16  & 0.31 & 0.15   & 0.75   & 0.58  & 0.36 & 1.00    \\ \hline
4.                              & turn  & on   & the    & faucet &       &      &         \\ 
                                & 0.94  & 1.00 & 0.44   & 0.87   &       &      &         \\ \hline
5.                              & slide & the  & green  & lever  & to    & the  & left    \\ 
                                & 0.52  & 0.23 & 0.94   & 1.00   & 0.77  & 0.30 & 0.78    \\ \hline
6.                              & open  & the  & window &        &       &      &         \\ 
                                & 0.83  & 0.32 & 1.00   &        &       &      &         \\ \hline
\end{tabular}
}
    \end{minipage}%
    \hfill
    \begin{minipage}{.38\linewidth}
      \centering
        \caption{Comparison of various ablations to the Dense+RGR model. }
\resizebox{\columnwidth}{!}{
\begin{tabular}{lrr}
\hline
\multicolumn{1}{c}{\textbf{Setting}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Mean\\ Successful\\ Episodes\end{tabular}}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}p-value\\ w.r.t.\\ Dense\end{tabular}}} \\ \hline %\hline
Dense                          & 79.4               & -                     \\ %\hline
Dense+RGR                      & 126.9              & 0.0340                \\ \hline %\hline
LastFrame                      & 133.5              & 0.0114                \\ %\hline
MeanpoolLang                   & 138.3              & 0.0004                \\ %\hline
MeanpoolTraj                   & 78.4               & 0.9601                \\ %\hline
SingleView                     & 100.4              & 0.3789                \\ %\hline
Dense+CLS                      & 102.0              & 0.6384                \\ \hline
\end{tabular}
}
    \end{minipage} 
\end{table}

